Jetting Through The Primordial Universe

Collisions of heavy ion nuclei at relativistic speeds (close to the speed of light) creates a high temperature and very dense form of matter, now known to consist of de-confined quarks and gluons, named the quark gluon plasma (QGP). In this thesis, Run1 experimental data from pp and heavy ion collisions at the CERN LHC is analyzed with the CMS detector. The pp jet cross section is compared with next to leading order theoretical calculations supplemented with non perturbative corrections for three different jet radii highlighting better comparisons for larger radii jets. Measurement of the jet yield followed by the nuclear modification factors in proton-lead at 5.02 TeV and lead-lead collisions at 2.76 TeV are presented. A new data driven technique is introduced to estimate and correct for the fake jet contribution in PbPb for low transverse momenta jets. The nuclear modification factors studied in this thesis show jet quenching to be attributed to final state effects, have a strong correlation to the event centrality, a weak inverse correlation to the jet transverse momenta and an apparent independence on the jet radii in the kinematic range studied. These measurements are compared with leading theoretical model calculations and other experimental results at the LHC leading to unanimous agreement on the qualitative nature of jet quenching. This thesis also features novel updates to the Monte Carlo heavy ion event generator JEWEL (Jet Evolution With Energy Loss) including the boson-jet production channels and also background subtraction techniques to reduce the effect of the thermal background. Keeping track of these jet-medium recoils in JEWEL due to the background subtraction techniques significantly improves its descriptions of several jet structure and sub-structure measurements at the LHC. [Shortened abstract]

==> acknowledgements_test.tex <==
TO BE ADDED

==> app4.tex <==
	
	\begin{figure}[h]
	   \centering
	   \includegraphics[width=0.45\textwidth]{Figures/app4/responseMatrix} 
	   \includegraphics[width=0.45\textwidth]{Figures/app4/mc_closure} 
	   \caption{Left: Mid rapidity jet \pt response matrix derived from PYTHIA+HIJING. Right: Unfolding closure test}
	   \label{fig:pPbresponseMatrixClosure}
	\end{figure}
	
